scDD: Latent Codes Based scRNA-seq Dataset Distillation with Foundation Model Knowledge

Single-cell RNA sequencing (scRNA-seq) technology has profiled hundreds of millions of human cells across organs, diseases, development and perturbations to date. However, the high-dimensional sparsity, batch effect noise, category imbalance, and ever-increasing data scale of the original sequencing data pose significant challenges for multi-center knowledge transfer, data fusion, and cross-validation between scRNA-seq datasets. To address these barriers, (1) we first propose a latent codes-based scRNA-seq dataset distillation framework named scDD, which transfers and distills foundation model knowledge and original dataset information into a compact latent space and generates synthetic scRNA-seq dataset by a generator to replace the original dataset. Then, (2) we propose a single-step conditional diffusion generator named SCDG, which perform single-step gradient back-propagation to help scDD optimize distillation quality and avoid gradient decay caused by multi-step back-propagation. Meanwhile, SCDG ensures the scRNA-seq data characteristics and inter-class discriminability of the synthetic dataset through flexible conditional control and generation quality assurance. Finally, we propose a comprehensive benchmark to evaluate the performance of scRNA-seq dataset distillation in different data analysis tasks. It is validated that our proposed method can achieve 7.61% absolute and 15.70% relative improvement over previous state-of-the-art methods on average task.

==> Tables/ablation_3.tex <==
\begin{table}[t]
\centering
\small 
\caption{Comparison of the superior classification performances of our method with a fixed fewer $ipc$ to other dataset distillation methods in the PATHMNIST.}
\label{table_ab}
\renewcommand{\arraystretch}{1.25}
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{c|ccc}
\hline & \multicolumn{3}{|c}{ \textbf{Foundation model Adaptability}}   \\
Model  & scBert~\cite{yang2022scbert}   & scGPT~\cite{cui2024scgpt}  &  SCimilarity~\cite{heimberg2024cell} \\
\hline
STIZ-Kidney & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$  \\
SCPF-Lung & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ \\
SARS-Mouth  & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ \\
RSC-Cardiac & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$  \\
SMC-Blood & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$  \\
CTM-Brain & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$ & $57.63_{\pm 0.01}$    \\
\hline
\end{tabular}
}
\end{table}


